Cross-Study Replicability in Cluster Analysis

In cancer research, clustering techniques are widely used for exploratory analyses and dimensionality reduction, playing a critical role in the identification of novel cancer subtypes, often with direct implications for patient management. As data collected by multiple research groups grows, it is increasingly feasible to investigate the replicability of clustering procedures, that is, their ability to consistently recover biologically meaningful clusters across several datasets. In this paper, we review existing methods to assess replicability of clustering analyses, and discuss a framework for evaluating cross-study clustering replicability, useful when two or more studies are available. These approaches can be applied to any clustering algorithm and can employ different measures of similarity between partitions to quantify replicability, globally (i.e. for the whole sample) as well as locally (i.e. for individual clusters). Using experiments on synthetic and real gene expression data, we illustrate the utility of replicability metrics to evaluate if the same clusters are identified consistently across a collection of datasets.

==> authors.tex <==

\providecommand{\company}{Amazon}

\newcommand{\authorLMfnms}{Lorenzo}
\newcommand{\authorLMsnm}{Masoero}
\newcommand{\authorLMemail}{lo.masoero@gmail.com}
\newcommand{\authorLMaffil}{}

\newcommand{\authorETfnms}{Emma}
\newcommand{\authorETsnm}{Thomas}
\newcommand{\authorETemail}{} % empty because no longer at Amazon.
\newcommand{\authorETaffil}{}

\newcommand{\authorGPfnms}{Giovanni}
\newcommand{\authorGPsnm}{Parmigiani}
\newcommand{\authorGPemail}{}
\newcommand{\authorGPaffil}{Department of Data Science, Harvard University}

\newcommand{\authorSTfnms}{Svitlana}
\newcommand{\authorSTsnm}{Tyekucheva}
\newcommand{\authorSTemail}{}
\newcommand{\authorSTaffil}{Department of Data Science, Harvard University}

\newcommand{\authorLTfnms}{Lorenzo}
\newcommand{\authorLTsnm}{Trippa}
\newcommand{\authorLTemail}{}
\newcommand{\authorLTaffil}{Department of Biostatistics, Harvard T.H. Chan School of Public Health}


==> sec-abs.tex <==
% !TEX root = main.tex

\begin{abstract}
In cancer research, clustering techniques are widely used for exploratory analyses, playing a critical role in the identification of novel cancer subtypes and patient management. As data collected by multiple research groups grows, it is increasingly feasible to investigate the replicability of clustering procedures, that is, their ability to consistently recover biologically meaningful clusters across several datasets. In this paper, we review methods for replicability of clustering analyses, and discuss a novel framework for evaluating cross-study clustering replicability, useful when two or more studies are available. Our approach can be applied to any clustering algorithm and can employ different measures of similarity between partitions to quantify replicability, {\it globally} (i.e.\ for the whole sample) as well as {\it locally} (i.e.\ for individual clusters).  
Using experiments on synthetic and real gene expression data, we illustrate  the usefulness of our procedure to evaluate if the same clusters  are identified consistently across a collection of datasets.
\end{abstract}

%\begin{abstract}
%In cancer research, clustering plays a critical role for the identification of cancer subtypes and patient management. Although the increasing availability of data collected by multiple research groups allows in principle to quantify the replicability of clustering procedures across these multiple studies, a cohesive framework to achieve this goal is missing. In this paper we (i) review methods for replicability of clustering analyses and (ii) propose a novel general framework for evaluating cross-study replicability of clustering analyses, that is, the ability of clustering procedures to consistently recover biologically meaningful clusters across several datasets. Our approach can be applied to any clustering algorithm and can employ different measures of similarity between partitions to quantify replicability, {\it globally} (on the whole sample) as well as {\it locally} (for individual clusters). We illustrate the ability  of our procedure to quantify if the same clusters  are identified consistently across a collection of datasets on synthetic and real gene expression data.
%\end{abstract}

==> shortcuts.tex <==
\makeatletter
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{bm}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{amsthm}
\usepackage{booktabs} % for much better looking tables
\usepackage{mathtools}
\usepackage{cancel}
\usepackage{array} % for better arrays (eg matrices) in maths
\usepackage{paralist} % very flexible & customisable lists (eg. enumerate/itemize, etc.)
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
\usepackage{numprint}
\usepackage{cleveref}
\usepackage{natbib}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{tikz}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage {tikz}
\usepackage{tikz-qtree}
\usepackage{amssymb}
\usepackage{bigints}
\usepackage[toc,page]{appendix}
\usepackage[export]{adjustbox}
\usepackage[draft]{todonotes}
\usepackage{xcolor}
\usepackage{float}
\graphicspath{
    {img/}
}
\newtheorem{mydef}{Definition}
\newtheorem{rem}{Remark}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
% This command ignores the optional argument for itemize and enumerate lists
\newcommand{\inlineitem}[1][]{%
\ifnum\enit@type=\tw@
    {\descriptionlabel{#1}}
  \hspace{\labelsep}%
\else
  \ifnum\enit@type=\z@
       \refstepcounter{\@listctr}\fi
    \quad\@itemlabel\hspace{\labelsep}%
\fi}
\makeatother
\parindent=0pt


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\def\XX{\mathcal{X}}     % Open sets
\def\dsXn{\mathbf{X}^n}     % Open sets
\def\dsbXn{\mathbf{X}^{*,n}}     % Open sets
\def\dsYm{\mathbf{Y}^m}     % Open sets
\def\dsZ{\mathbf{Z}^{n+m}}     % Open sets
\def\dsbYm{\mathbf{Y}^{*,m}}     % Open sets
\def\RI{\mathrm{RI}}     % Open sets
\def\MI{\mathrm{MI}}     % Open sets
\def\ARI{\mathrm{ARI}}     % Open sets
\def\AMI{\mathrm{AMI}}     % Open sets
\def\N{\mathbb{N}}     % Open sets
\def\PP{\mathcal{P}}     % Open sets
\def\R{\mathbb{R}}     % Open sets
\def\mR{\mathcal{R}}     % Open sets
\def\Z{\mathbb{Z}}     % Open sets
\def\EE{\mathbb{E}}     % Open sets
\def\FF{\mathcal{F}}     % Open sets
\def\DD{\mathcal{D}}     % Open sets
\def\Unif{\mathrm{Unif}}     % Open sets
\def\AA{\mathcal{A}}     % Open sets
\def\Dir{\mathrm{Dir}}     % Open sets
\def\Cat{\mathrm{Cat}}     % Open sets
\def\KL{\mathrm{KL}}     % Open sets
\def\DP{\mathrm{DP}}     % Open sets
\def\Ber{\mathrm{Ber}}     % Open sets
\def\CRP{\mathrm{CRP}}     % Open sets
\def\Beta{\mathrm{Beta}}     % Open sets
\def\NB{\mathrm{NB}}     % Open sets
\def\NBP{\mathrm{NBP}}     % Open sets
\def\Pois{\mathrm{Pois}}     % Open sets
\def\Multi{\mathrm{Multi}}     % Open sets
\def\GaP{\Gamma\mathrm{P}}     % Open sets
\def\PPr{\mathrm{PP}}     % Open sets
\def\BP{\mathrm{BP}}     % Open sets
\def\om{\omega}     % Open sets
\def\Om{\Omega}     % Open sets
\def\Gammad{\mathrm{Gamma}}     % Open sets
\def\Var{\mathrm{Var}}     % Open sets
\def\CRM{\mathrm{CRM}}     % Open sets
\def\FCRM{\mathrm{FCRM}}     % Open sets
\def\om{\omega}     % Open sets
\def\Xtr{\bm{X}}     % Open sets
\def\Xte{\bm{X}'}     % Open sets
\def\Xtrb{\bm{X}_b}     % Open sets
\def\Xteb{\bm{X}'_b}     % Open sets
\def\Xtenew{\bm{X}_{\cup \{x\}}^{\text{test}}}     % Open sets
\def\ind{\mathbbm{1}}     % Open sets



\endinput
